Deep Weighted Consensus: Dense correspondence confidence maps for 3D shape registration

We present a new paradigm for rigid alignment between point clouds based on learnable weighted consensus which is robust to noise as well as the full spectrum of the rotation group. Current models, learnable or axiomatic, work well for constrained orientations and limited noise levels, usually by an end-to-end learner or an iterative scheme. However, real-world tasks require us to deal with large rotations as well as outliers and all known models fail to deliver. Here we present a different direction. We claim that we can align point clouds out of sampled matched points according to confidence level derived from a dense, soft alignment map. The pipeline is differentiable, and converges under large rotations in the full spectrum of SO(3), even with high noise levels. We compared the network to recently presented methods such as DCP, PointNetLK, RPM-Net, PRnet, and axiomatic methods such as ICP and Go-ICP. We report here a fundamental boost in performance.

==> Sections/Deep Weighted Consensus/Confidence_based_consensus_problem.tex <==
\paragraph{Confidence based sampling}
The soft correspondence mapping defines a dense alignment between the shapes. DWC presents a differentiable reduction procedure from $\softP$ to the rigid alignment solution.
Here, unlike previous works that used all points in $\mathcal{X}$ \cite{dcp,pointnetlk}, or chose a fixed subset of points $\{x_i|x_i\in \mathcal{X}\}$ using a $top-k$ heuristic \cite{prnet}, we construct a categorical distribution over the source points, by which we sample points that participate in the solution to the alignment problem.

We define the \textit{confidence metric} $\softP_m$ to be :
\begin{equation}
    \softP_{m_i} = \max_j \softP_{i,j}.
\end{equation}

$\softP_{m} \in \mathbb{R}^{|\mathcal{X}|}$ is a proxy to the confidence level of $\mathcal{X}$ in $\pi(\mathcal{X})$, that is, for point $i$ where DWC has high certainty in the mapping, $\softP_{m_i}$ will be high, while for points where the network is not certain, $\softP_{m_i}$ will be low\footnote{While not common, for $\max_j \softP_{i,j}<0$ we set $\softP_{m_i}=0$.}. 

We normalize $\softP_m$: 
\begin{equation}
   \widehatmine{\softP_m} = \frac{\softP_{m}}{\sum\limits_{i=0}^{|\mathcal{X}|-1} \softP_{m_i}} 
\end{equation}
and define the confidence sampling distribution $S$ over the points in $\mathcal{X}$:

\begin{equation}
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{cc}
$x_i\in \{i|0\leq i < |\mathcal{X}|\}$ & Support\\[0.2cm]
$s_{X}(x_i)=S(X=x_i)=\widehatmine{\softP_{m_i}}$ & PMF
\end{tabular}%
}
\end{equation}
In what follows we explain how $S$ defines both the registration solution and the optimization objective.



==> Sections/Deep Weighted Consensus/Consensus_problem.tex <==
\paragraph{Confidence based consensus}\label{subsec:consensus}
Based on the confidence distribution over the source points $S$,
DWC samples $Q$\footnote{$|Q|$ is a hyper-parameter and was set to $\frac{|\mathcal{X}|}{10}$ in the experiments.} source points. These points are used both for the optimization of the dense alignment, and for the solution of the optimal $R,t$ parameters using the SVD decomposition.
Using the described formulation we allow the network to learn which are the most significant points for the matching and factor them accordingly.

At inference, we sample $k$ "experiment" groups from $Q$ uniformly, each with $r=|Q|/k$ points, where $r$ is the number of points fed to the alignment solver. By sampling uniformly from $Q$, each "experiment" is distributed according to $S$, the confidence based distribution.
We set the chamfer distance \cite{chamfer} between the target shape and the source shape after applying the inferred transformation as the evaluation metric. The extracted $R,t$ parameters for the experiment with the lowest chamfer distance are chosen as the transformation parameters.
Although our inference scheme can be seen as a weighted variant of RANSAC \cite{ransac}, a major difference is the fact that unlike previous methods that used RANSAC, our consensus voting is confident based, and takes part of the learning pipeline itself, and not only during test-time. The incorporation of our weighted consensus problem into the network leads to faster convergence and improved results, as demonstrated in the experiments (Section \ref{section:Experimentation}).

The fact that DWC performs $k$ separate experiments for $R,t$ is not only beneficial to achieving the highest score among all state-of-the-art methods but also provides a leap in performance due parallel computing utilization; solving $k$ $SV\!D$ problems with $m$ equations is up to two orders of magnitude faster than solving one $SV\!D$ problem with $kl$ equations, as done by \cite{prnet,dcp,pointnetlk}.

==> Sections/Deep Weighted Consensus/Deep_Weighted_Consensus.tex <==
\vspace{-5mm}
\section{Deep Weighted Consensus}
\vspace{-2mm}
Deep weighted consensus is a self-supervised deep network designed to solve the rigid alignment problem of 3D shapes.

In short, DWC extracts rotation-invariant features of the input point clouds, and builds local and global features for the two shapes. The fusion of these high-dimensional features define the \textit{soft correspondence mapping} between the shapes by computing the cosine-similarity of the features. Next, the network defines a probability distribution based on the certainty of each source point in its map, and sample confident points that partake in the consensus problem. At inference, DWC uses the sampled points to find the optimal $R,t$ (see figure \ref{fig:architecture_scheme} for illustration). 

\subsection{Method}
\input{Sections/Deep Weighted Consensus/Rotation invariant descriptors}

\input{Sections/Deep Weighted Consensus/Feature Extraction Network}

\input{Sections/Deep Weighted Consensus/Soft correspondence mapping}

\input{Sections/Deep Weighted Consensus/Confidence based consensus problem}

\input{Sections/Deep Weighted Consensus/Consensus problem}

\input{Sections/Deep Weighted Consensus/Loss}




==> Sections/Deep Weighted Consensus/Feature_Extraction_Network.tex <==
\paragraph*{Feature Extraction Network}\label{subsec:feature_gen}
The objective of the feature extraction network is to embed the unaligned input point clouds $\mathcal{X}$ and $\mathcal{Y}$ to a common high dimensional feature space. $FEN$ does this by combining two variants of DGCNN \cite{dgcnn}, namely the classification and segmentation networks, henceforth noted by $DGCNN_{glob},DGCNN_{loc}$ respectively. 
For both networks, we use the representations generated before the last aggregation function, and define them such that for point cloud $\mathcal{X}$ with $N$ points, the output features dimensions are $h_{loc}(\mathcal{X})\in \mathbb{R}^{N\times l_1}$ and 
$h_{glob}(\mathcal{X})\in \mathbb{R}^{l_2}$ where $l_1,l_2$ are network hyper-parameters.

As opposed to the original paper \cite{dgcnn} or subsequent works \cite{dcp,dvir3}, $FEN$ does not use the dynamically changing neighborhood of the graph when applying convolutions in deeper layers of the network, as it causes message passing between distinct parts of the graph, that may have similar characteristics. While this is a good quality for \textit{segmentation} networks, identifying graph-symmetries is crucial for solving the alignment problem. Numerically, we have found that this change improves results substantially (Section \ref{subsec:ablation}).

The final step of $FEN$ is to fuse the global and local features per point. Given $h_{glob}(\mathcal{X})$ and $h_{loc}(\mathcal{X})$, we concatenate the global feature with each local feature resulting in $h_{GL}\in \mathbb{R}^{N\times (l_1+l_2)}$, and propagate $h_{GL}$ through a series of dense non-linear layers, resulting in $\hat{h}_{\mathcal{X}}\in \mathbb{R}^{N\times l_3}$. We mark the Global-Local-Fusion process by GLF.
A detailed layout of $FEN$ is provided in the supplementary.


==> Sections/Deep Weighted Consensus/Loss.tex <==
\subsection{Loss}\label{subsec:losses}


DWC optimizes the feature correlation directly by presenting three constraints on the soft correspondence matrix.
During our self-supervised training, each source shape is being augmented by rotation, translation, and noise. As the same points are "chosen" for both source $\mathcal{X}$ and target $\mathcal{Y}$, the dense mapping is the identity map $\pi(\mathcal{X}_i)=\mathcal{Y}_i$ .
We use this observation to define $\mathcal{L}_h$, the hard mapping loss:
\begin{equation}
\mathcal{L}_h = \frac{1}{|\mathcal{X}|}\sum_{i=0}^{|\mathcal{X}|-1}(1-\softP_{ii})
\end{equation}
which strives to have the cosine similarity between $x_i$,$y_i$ equal 1, de facto teaching the network to be invariant to the augmentation presented.

Furthermore, DWC presents a novel contrastive loss that motivates the embedding of a source point $x_i$ to be close to the neighbors of the corresponding target point $y_i$, while far from the points not in $y_i$'s proximity.
The neighborhood $\mathcal{N}$ of $y_i$ is defined to be its $k$ Euclidian nearest neighbors.
Defined by $A$ is the adjacency matrix of the target shape induced by $\mathcal{N}$ such that:
\begin{equation}
	A_{ij} = 1 \Leftrightarrow y_j \in \mathcal{N}_i
\end{equation}
We define $\overline{A}$ to be the negation of $A$, where $\overline{A}_{ij}=1$  for non-neighbors and $\overline{A}_{ij}=0$ otherwise.
Using the above notation, the positive $\mathcal{L}_{p}$ and negative $\mathcal{L}_{n} $ contrastive losses per-point are:
\begin{align}
\mathcal{L}_{p_{i}}=\sum_{\{j| A_{ij}=1\}}\max (0,m_p-\softP_{ij})\\
\mathcal{L}_{n_{i}}=\sum_{\{j| \overline{A}_{ij}=1\}}\max(0,\softP_{ij}-m_n)
\end{align}


Where $m_p$ and $m_n$ are the positive and negative margins.
The contrastive loss incorporates two significant advantages over previous methods:
\begin{itemize}
\item By applying the contrastive loss we fuse the topology of the graphs not only to the learning process but to the objective function itself.
\item As all target points takes part in $\mathcal{L}_{n}$, the network is exposed to all points, and not only to a chosen subset.
\end{itemize}
We further define $w_{Q_i}$ as the number of times $\mathcal{X}_i$ was chosen by $Q$

\begin{equation}
    w_{Q_i}=\sum_{j=1}^{|Q|}[Q_j=\mathcal{X}_i]
\end{equation} and factor the contrastive loss of $\mathcal{X}_i$ accordingly
\begin{align}
\mathcal{L}_{pQ}=\frac{1}{|Q|\sum\limits_{i,j} A_{ij}} \sum_{i}^{|\mathcal{X}|}w_{Q_i}\mathcal{L}_{p_{i}}\\
\mathcal{L}_{nQ}=\frac{1}{|Q|\sum\limits_{i,j} \overline{A}_{ij}} \sum_{i}^{|\mathcal{X}|}w_{Q_i}\mathcal{L}_{n_{i}}
\end{align}
By integrating $w_{Q_i}$ into $\mathcal{L}_{[n,p]}$ the contrastive loss is weighted based on the confidence of each source point. $\mathcal{L}_{[n,p] Q}$ compels DWC to define points as confident only if they are similar to the neighborhood of their matched target point, increasing the chances they are good "anchor" points for the alignment solution.

The final optimization function of DWC is:
\begin{equation}
 \mathcal{L}_C = \mathcal{L}_{h} + \mathcal{L}_{pQ} + \mathcal{L}_{nQ}
\end{equation}


==> Sections/Deep Weighted Consensus/Rotation_invariant_descriptors.tex <==
\paragraph{Rotation invariant descriptors}\label{subsec:rot_inv_feat}
The first step of the DWC pipeline is to extract rotation-invariant ($RI$) descriptors out of the Euclidean coordinates of the input point clouds. These features are the input descriptors for the Feature Extractor Network ($FEN$).
The registration problem in the full range of SO(3) is hard and state-of-the-art methods such as \cite{dgcnn,pointcnn,sonet} fail to generate meaningful representations under such deformations, as proven in \cite{rot1,rot2} and demonstrated in the experimentation shown in section \ref{section:Experimentation}.

One reason for the struggle of networks using the Euclidean coordinates as the inputs for the $FEN$ is the predicted transformation output for symmetric shapes. On symmetric shapes transformed by a $~180\degree$ rotation, such networks will suggest the exact opposite transformation to the correct rotation, as locally, symmetric parts have identical embeddings given the same input features. Illustration to the phenomena can be seen in the plane example in figure \ref{fig:Tizer_pairs}.

Inspired by the local rotation invariant features presented in \cite{rot1}, we present global and local $RI$ features for every point $x$ conditioned by the neighborhood of a source point $m$, which for point clouds is usually the $k$-nearest neighbors.

Our features do not need normal approximations as \cite{rot3}, or geometric median computation as \cite{rot2}, hence are suitable for real-time applications as demonstrated in the timing evaluation provided in the supplementary.\\
Given the Euclidean center of the point cloud $O$, a source point $p$ of neighborhood $\mathcal{N}_p$, and $m$, the Euclidean center of $\mathcal{N}_p$, the rotation invariant descriptors of $x\in \mathcal{N}_p$ are:
\begin{table}[H]
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{l|l}
\multicolumn{1}{c|}{Local} & \multicolumn{1}{c}{Global} \\
 $\alpha_{xmp}=\angle(\vv{mx},\vv{mp})$ & $\alpha_{xOp}=\angle(\vv{Ox},\vv{Op})$
 \\
 $\alpha_{xpm}=\angle(\vv{px},\vv{pm})$ & 
 $\alpha_{xOm}=\angle(\vv{Ox},\vv{Om})$
 \\
 $d(x,m)=||x-m||_{2}$     &   $d(x,O)=||x-O||_{2}$     \\
 $d(x,p)=||x-p||_{2}$     &        \\
  
\end{tabular}%
}
\end{table}
\noindent  Where $\vv{aa'}$ is the vector from $a$ to $a'$ in the 3D space and $\angle{(\vv{ab},\vv{ac})}$ is the angle between $\vv{ab}$ and $\vv{ac}$.\\
The aggregated $RI$ feature is:
\begin{align}\label{eq:ri_features}
\begin{split}
    f_{\mathcal{N}_p}(x)=[&\alpha_{xmp},\alpha_{xpm},d(x,m),d(x,p),\\&\alpha_{xOp},\alpha_{xOm},d(x,O)]
\end{split}
\end{align}


We exemplify the significance of using the $RI$ features in the results (Section \ref{subsec:modelnet}) as well as in the ablation study (Section \ref{subsec:ablation}).



==> Sections/Deep Weighted Consensus/Soft_correspondence_mapping.tex <==
\paragraph{Soft correspondence mapping}\label{subsec:softcorr}
DWC has the ability to match key points that are similar between $\mathcal{X}$ and $\mathcal{Y}$ with high probability and extract the transformation using these points. Therefore, DWC avoids using outliers in the transformation computation with high probability, in contrast to previous works \cite{dcp,pointnetlk}.
To find these keypoints we define the soft correspondence mapping $\mathcal{P}$, which is given by the cosine similarity of the latent representations of $\hat{h}_{\mathcal{X}}, \hat{h}_{\mathcal{Y}}$: 
\begin{equation}
  \softP_{i,j}=\frac{ \hat{h}_{\mathcal{X}_i} \cdot \hat{h}_{\mathcal{Y}_j}} {|| \hat{h}_{\mathcal{X}_i} ||_2 \cdot ||\hat{h}_{\mathcal{Y}_j}||_2}
\end{equation}
 
$\softP$ is a pseudo\footnote{$\softP$ contains negative values and the rows do not sum to 1.} probability matrix, where $\softP_{ij}$ can be interpreted as the probability that $\mathcal{X}_i$ corresponds to $\mathcal{Y}_j$.\\
Using $\softP$ we define the point-wise mapping between the source and target shapes $\pi: \mathcal{X} \rightarrow \mathcal{Y}$ to be: 
\begin{equation}
    \pi(\mathcal{X}_i)=\argmax_j \softP_{ij}.
\end{equation}
In the theoretical case of perfect samples, given 3 non-collinear points that are correctly matched between the graphs by $\pi(\mathcal{X})$, a closed-form solution to the problem is feasible. In the case of noise and outliers in the mapping, an optimal solution in the least-squares sense was suggested in the Kabsch algorithm \cite{rtsolve}, which solves for $R,t$ given the singular value decomposition of $\pi(\mathcal{X})$.

In the paragraphs that follow, we explain how a sampling procedure based on $\softP$ defines the subset of points that we use as input to the Kabsch algorithm.


==> Sections/Summary and Limitations/Summary_and_Limitations.tex <==

\section{Summary}
\label{sec:Summary and Limitations}

DWC offers a paradigm shift for solving the rigid alignment problem by explicitly optimizing the dense map. In addition, unlike previous methods that solved for the globally optimal parameters which tend to be extremely sensitive to outliers, DWC presents a differentiable reduction procedure based on the confidence of each source point in its correspondence map, and weight the alignment solution accordingly. We exemplify under multiple experiments how these novelties present a significant boost in performance in all popular benchmarks, and, for the first time, solve the alignment problem for extreme rigid transformations in the full spectrum of SO(3). 



==> eso-pic.sty.tex <==
%%
%% This is file `eso-pic.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% eso-pic.dtx  (with options: `package')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 1998-2002 by Rolf Niepraschk <niepraschk@ptb.de>
%% 
%% This file may be distributed and/or modified under the conditions of
%% the LaTeX Project Public License, either version 1.2 of this license
%% or (at your option) any later version.  The latest version of this
%% license is in:
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of LaTeX version
%% 1999/12/01 or later.
%% 
\NeedsTeXFormat{LaTeX2e}[1999/12/01]
\ProvidesPackage{eso-pic}
   [2002/11/16 v1.1b eso-pic (RN)]
\input{iccv_eso.sty}
\newcommand\LenToUnit[1]{#1\@gobble}

\newcommand\AtPageUpperLeft[1]{%
  \begingroup
    \@tempdima=0pt\relax\@tempdimb=\ESO@yoffsetI\relax
    \put(\LenToUnit{\@tempdima},\LenToUnit{\@tempdimb}){#1}%
  \endgroup
}
\newcommand\AtPageLowerLeft[1]{\AtPageUpperLeft{%
  \put(0,\LenToUnit{-\paperheight}){#1}}}
\newcommand\AtPageCenter[1]{\AtPageUpperLeft{%
  \put(\LenToUnit{.5\paperwidth},\LenToUnit{-.5\paperheight}){#1}}%
}
\newcommand\AtTextUpperLeft[1]{%
  \begingroup
    \setlength\@tempdima{1in}%
    \ifodd\c@page%
      \advance\@tempdima\oddsidemargin%
    \else%
      \advance\@tempdima\evensidemargin%
    \fi%
    \@tempdimb=\ESO@yoffsetI\relax\advance\@tempdimb-1in\relax%
    \advance\@tempdimb-\topmargin%
    \advance\@tempdimb-\headheight\advance\@tempdimb-\headsep%
    \put(\LenToUnit{\@tempdima},\LenToUnit{\@tempdimb}){#1}%
  \endgroup
}
\newcommand\AtTextLowerLeft[1]{\AtTextUpperLeft{%
  \put(0,\LenToUnit{-\textheight}){#1}}}
\newcommand\AtTextCenter[1]{\AtTextUpperLeft{%
  \put(\LenToUnit{.5\textwidth},\LenToUnit{-.5\textheight}){#1}}}
\newcommand{\ESO@HookI}{} \newcommand{\ESO@HookII}{}
\newcommand{\ESO@HookIII}{}
\newcommand{\AddToShipoutPicture}{%
  \@ifstar{\g@addto@macro\ESO@HookII}{\g@addto@macro\ESO@HookI}}
\newcommand{\ClearShipoutPicture}{\global\let\ESO@HookI\@empty}
\newcommand\ESO@isMEMOIR[1]{}
\@ifclassloaded{memoir}{\renewcommand\ESO@isMEMOIR[1]{#1}}{}
\newcommand{\@ShipoutPicture}{%
  \bgroup
    \@tempswafalse%
    \ifx\ESO@HookI\@empty\else\@tempswatrue\fi%
    \ifx\ESO@HookII\@empty\else\@tempswatrue\fi%
    \ifx\ESO@HookIII\@empty\else\@tempswatrue\fi%
    \if@tempswa%
      \@tempdima=1in\@tempdimb=-\@tempdima%
      \advance\@tempdimb\ESO@yoffsetI%
      \ESO@isMEMOIR{%
        \advance\@tempdima\trimedge%
        \advance\@tempdima\paperwidth%
        \advance\@tempdima-\stockwidth%
        \if@twoside\ifodd\c@page\else%
          \advance\@tempdima-2\trimedge%
          \advance\@tempdima-\paperwidth%
          \advance\@tempdima\stockwidth%
        \fi\fi%
        \advance\@tempdimb\trimtop}%
      \unitlength=1pt%
      \global\setbox\@cclv\vbox{%
        \vbox{\let\protect\relax
          \pictur@(0,0)(\strip@pt\@tempdima,\strip@pt\@tempdimb)%
            \ESO@HookIII\ESO@HookI\ESO@HookII%
            \global\let\ESO@HookII\@empty%
          \endpicture}%
          \nointerlineskip%
        \box\@cclv}%
    \fi
  \egroup
}
\EveryShipout{\@ShipoutPicture}
\RequirePackage{keyval}
\newif\ifESO@dvips\ESO@dvipsfalse \newif\ifESO@grid\ESO@gridfalse
\newif\ifESO@texcoord\ESO@texcoordfalse
\newcommand*\ESO@gridunitname{}
\newcommand*\ESO@gridunit{}
\newcommand*\ESO@labelfactor{}
\newcommand*\ESO@griddelta{}\newcommand*\ESO@griddeltaY{}
\newcommand*\ESO@gridDelta{}\newcommand*\ESO@gridDeltaY{}
\newcommand*\ESO@gridcolor{}
\newcommand*\ESO@subgridcolor{}
\newcommand*\ESO@subgridstyle{dotted}% ???
\newcommand*\ESO@gap{}
\newcommand*\ESO@yoffsetI{}\newcommand*\ESO@yoffsetII{}
\newcommand*\ESO@gridlines{\thinlines}
\newcommand*\ESO@subgridlines{\thinlines}
\newcommand*\ESO@hline[1]{\ESO@subgridlines\line(1,0){#1}}
\newcommand*\ESO@vline[1]{\ESO@subgridlines\line(0,1){#1}}
\newcommand*\ESO@Hline[1]{\ESO@gridlines\line(1,0){#1}}
\newcommand*\ESO@Vline[1]{\ESO@gridlines\line(0,1){#1}}
\newcommand\ESO@fcolorbox[4][]{\fbox{#4}}
\newcommand\ESO@color[1]{}
\newcommand\ESO@colorbox[3][]{%
  \begingroup
    \fboxrule=0pt\fbox{#3}%
  \endgroup
}
\newcommand\gridSetup[6][]{%
  \edef\ESO@gridunitname{#1}\edef\ESO@gridunit{#2}
  \edef\ESO@labelfactor{#3}\edef\ESO@griddelta{#4}
  \edef\ESO@gridDelta{#5}\edef\ESO@gap{#6}}
\define@key{ESO}{texcoord}[true]{\csname ESO@texcoord#1\endcsname}
\define@key{ESO}{pscoord}[true]{\csname @tempswa#1\endcsname
  \if@tempswa\ESO@texcoordfalse\else\ESO@texcoordtrue\fi}
\define@key{ESO}{dvips}[true]{\csname ESO@dvips#1\endcsname}
\define@key{ESO}{grid}[true]{\csname ESO@grid#1\endcsname
  \setkeys{ESO}{gridcolor=black,subgridcolor=black}}
\define@key{ESO}{colorgrid}[true]{\csname ESO@grid#1\endcsname
  \setkeys{ESO}{gridcolor=red,subgridcolor=green}}
\define@key{ESO}{gridcolor}{\def\ESO@gridcolor{#1}}
\define@key{ESO}{subgridcolor}{\def\ESO@subgridcolor{#1}}
\define@key{ESO}{subgridstyle}{\def\ESO@subgridstyle{#1}}%
\define@key{ESO}{gridunit}{%
  \def\@tempa{#1}
  \def\@tempb{bp}
  \ifx\@tempa\@tempb
    \gridSetup[\@tempa]{1bp}{1}{10}{50}{2}
  \else
    \def\@tempb{pt}
    \ifx\@tempa\@tempb
      \gridSetup[\@tempa]{1pt}{1}{10}{50}{2}
    \else
      \def\@tempb{in}
      \ifx\@tempa\@tempb
        \gridSetup[\@tempa]{.1in}{.1}{2}{10}{.5}
      \else
        \gridSetup[mm]{1mm}{1}{5}{20}{1}
      \fi
    \fi
  \fi
}
\setkeys{ESO}{subgridstyle=solid,pscoord=true,gridunit=mm}
\def\ProcessOptionsWithKV#1{%
  \let\@tempc\@empty
  \@for\CurrentOption:=\@classoptionslist\do{%
    \@ifundefined{KV@#1@\CurrentOption}%
    {}{\edef\@tempc{\@tempc,\CurrentOption,}}}%
  \edef\@tempc{%
    \noexpand\setkeys{#1}{\@tempc\@ptionlist{\@currname.\@currext}}}%
  \@tempc
  \AtEndOfPackage{\let\@unprocessedoptions\relax}}%
\ProcessOptionsWithKV{ESO}%
\newcommand\ESO@div[2]{%
  \@tempdima=#1\relax\@tempdimb=\ESO@gridunit\relax
  \@tempdimb=#2\@tempdimb\divide\@tempdima by \@tempdimb%
  \@tempcnta\@tempdima\advance\@tempcnta\@ne}
\AtBeginDocument{%
  \IfFileExists{color.sty}
  {%
    \RequirePackage{color}
    \let\ESO@color=\color\let\ESO@colorbox=\colorbox
    \let\ESO@fcolorbox=\fcolorbox
  }{}
  \@ifundefined{Gin@driver}{}%
  {%
    \ifx\Gin@driver\@empty\else%
      \filename@parse{\Gin@driver}\def\reserved@a{dvips}%
      \ifx\filename@base\reserved@a\ESO@dvipstrue\fi%
    \fi
  }%
  \ifx\pdfoutput\undefined\else
    \ifx\pdfoutput\relax\else
      \ifcase\pdfoutput\else
        \ESO@dvipsfalse%
      \fi
    \fi
  \fi
  \ifESO@dvips\def\@tempb{eepic}\else\def\@tempb{epic}\fi
  \def\@tempa{dotted}%\def\ESO@gap{\LenToUnit{6\@wholewidth}}%
  \ifx\@tempa\ESO@subgridstyle
    \IfFileExists{\@tempb.sty}%
    {%
      \RequirePackage{\@tempb}
      \renewcommand*\ESO@hline[1]{\ESO@subgridlines\dottedline{\ESO@gap}%
        (0,0)(##1,0)}
      \renewcommand*\ESO@vline[1]{\ESO@subgridlines\dottedline{\ESO@gap}%
        (0,0)(0,##1)}
    }{}
  \else
    \ifx\ESO@gridcolor\ESO@subgridcolor%
      \renewcommand*\ESO@gridlines{\thicklines}
    \fi
  \fi
}
\ifESO@texcoord
  \def\ESO@yoffsetI{0pt}\def\ESO@yoffsetII{-\paperheight}
  \edef\ESO@griddeltaY{-\ESO@griddelta}\edef\ESO@gridDeltaY{-\ESO@gridDelta}
\else
  \def\ESO@yoffsetI{\paperheight}\def\ESO@yoffsetII{0pt}
  \edef\ESO@griddeltaY{\ESO@griddelta}\edef\ESO@gridDeltaY{\ESO@gridDelta}
\fi
\newcommand\ESO@gridpicture{%
  \begingroup
    \setlength\unitlength{\ESO@gridunit}%
    \ESO@color{\ESO@subgridcolor}%
    \ESO@div{\paperheight}{\ESO@griddelta}%
    \multiput(0,0)(0,\ESO@griddeltaY){\@tempcnta}%
      {\ESO@hline{\LenToUnit{\paperwidth}}}%
    \ESO@div{\paperwidth}{\ESO@griddelta}%
    \multiput(0,\LenToUnit{\ESO@yoffsetII})(\ESO@griddelta,0){\@tempcnta}%
      {\ESO@vline{\LenToUnit{\paperheight}}}%
    \ESO@color{\ESO@gridcolor}%
    \ESO@div{\paperheight}{\ESO@gridDelta}%
    \multiput(0,0)(0,\ESO@gridDeltaY){\@tempcnta}%
      {\ESO@Hline{\LenToUnit{\paperwidth}}}%
    \ESO@div{\paperwidth}{\ESO@gridDelta}%
    \multiput(0,\LenToUnit{\ESO@yoffsetII})(\ESO@gridDelta,0){\@tempcnta}%
      {\ESO@Vline{\LenToUnit{\paperheight}}}%
    \fontsize{10}{12}\normalfont%
    \ESO@div{\paperwidth}{\ESO@gridDelta}%
    \multiput(0,\ESO@gridDeltaY)(\ESO@gridDelta,0){\@tempcnta}{%
      \@tempcntb=\@tempcnta\advance\@tempcntb-\@multicnt%
      \ifnum\@tempcntb>1\relax
        \multiply\@tempcntb by \ESO@gridDelta\relax%
        \@tempdima=\@tempcntb sp\@tempdima=\ESO@labelfactor\@tempdima%
        \@tempcntb=\@tempdima%
        \makebox(0,0)[c]{\ESO@colorbox{white}{\the\@tempcntb}}%
      \fi}%
    \ifx\ESO@gridunitname\@empty\def\@tempa{0}\else\def\@tempa{1}\fi%
    \ESO@div{\paperheight}{\ESO@gridDelta}%
    \multiput(\ESO@gridDelta,0)(0,\ESO@gridDeltaY){\@tempcnta}{%
      \@tempcntb=\@tempcnta\advance\@tempcntb-\@multicnt%
      \ifnum\@tempcntb>\@tempa\relax
        \multiply\@tempcntb by \ESO@gridDelta\relax%
        \@tempdima=\@tempcntb sp\@tempdima=\ESO@labelfactor\@tempdima%
        \@tempcntb=\@tempdima%
        \makebox(0,0)[c]{\ESO@colorbox{white}{\the\@tempcntb}}%
      \fi
    }%
    \ifx\ESO@gridunitname\@empty\else%
      \thicklines\fboxrule=\@wholewidth%
      \put(\ESO@gridDelta,\ESO@gridDeltaY){\makebox(0,0)[c]{%
        \ESO@fcolorbox{\ESO@gridcolor}{white}{%
          \textbf{\ESO@gridunitname}}}}%
    \fi
    \normalcolor%
  \endgroup
}
\ifESO@grid\g@addto@macro\ESO@HookIII{\ESO@gridpicture}\fi
\endinput
%%
%% End of file `eso-pic.sty'.


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
